LLM-Personalize: Aligning LLM Planners with Human Preferences via Reinforced Self-Training for Housekeeping Robots

Large language models (LLMs) have shown significant potential for robotics applications, particularly task planning, by harnessing their language comprehension and text generation capabilities. However, in applications such as household robotics, a critical gap remains in the personalization of these models to individual user preferences. We introduce LLM-Personalize, a novel framework with an optimization pipeline designed to personalize LLM planners for household robotics. Our LLM-Personalize framework features an LLM planner that performs iterative planning in multi-room, partially-observable household scenarios, making use of a scene graph constructed with local observations. The generated plan consists of a sequence of high-level actions which are subsequently executed by a controller. Central to our approach is the optimization pipeline, which combines imitation learning and iterative self-training to personalize the LLM planner. In particular, the imitation learning phase performs initial LLM alignment from demonstrations, and bootstraps the model to facilitate effective iterative self-training, which further explores and aligns the model to user preferences. We evaluate LLM-Personalize on Housekeep, a challenging simulated real-world 3D benchmark for household rearrangements, and show that LLM-Personalize achieves more than a 30 percent increase in success rate over existing LLM planners, showcasing significantly improved alignment with human preferences. Project page: https://gdg94.github.io/projectllmpersonalize/.

==> table_correct_wrong.tex <==
\begin{table}[t]
\caption{Ablation: Correct vs. wrong placement steps (\textbf{Boldface}: highest \# correct steps, \underline{Underline}: lowest \# wrong steps across task set, \textbf{SI}: self-imitation, \textbf{IL}: imitation learning)}
    \scriptsize
    \setlength\tabcolsep{0.5pt}
\hspace*{-1cm}
\begin{tabular}{@{}ccccccccccccccccc@{}}
\toprule
\textbf{Scene ID} & \multicolumn{4}{c}{\textbf{Scene 1}} & \multicolumn{4}{c}{\textbf{Scene 2}} & \multicolumn{4}{c}{\textbf{Scene 3}} & \multicolumn{4}{c}{\textbf{Scene 4}} \\ \midrule
\textbf{task set} & \multicolumn{2}{c}{\textit{\textbf{test}}} & \multicolumn{2}{c}{\textit{\textbf{train}}} & \multicolumn{2}{c}{\textit{\textbf{test}}} & \multicolumn{2}{c}{\textit{\textbf{train}}} & \multicolumn{2}{c}{\textit{\textbf{test}}} & \multicolumn{2}{c}{\textit{\textbf{train}}} & \multicolumn{2}{c}{\textit{\textbf{test}}} & \multicolumn{2}{c}{\textit{\textbf{train}}} \\ \midrule
\textbf{✓/✗ Placements} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} & \textbf{✓} & \textbf{✗} \\ \midrule
\textbf{LLM-Planner} & 2.00 & 2.76 & 0.88 & 3.68 & 1.48 & 2.92 & 1.72 & 2.52 & 0.36 & 5.60 & 0.48 & 6.92 & 1.92 & 3.04 & 1.80 & 3.08 \\ \midrule
\textbf{LLM-Personalize(\il{})} & 3.00 & {\ul 1.64} & 1.45 & 1.56 & 8.12 & 1.48 & 2.36 & 3.74 & 1.24 & {\ul 1.12} & 1.21 & {\ul 1.26} & \textbf{6.24} & {\ul 2.72} & 3.80 & {\ul 2.73} \\ \midrule
\textbf{LLM-Personalize(\si1)} & \textbf{5.44} & 2.48 & 4.89 & 1.63 & \textbf{9.92} & {\ul 1.36} & \textbf{7.45} & {\ul 2.29} & \textbf{11.32} & 4.56 & \textbf{9.31} & 4.50 & 4.48 & 3.72 & 5.13 & 3.89 \\ \midrule
\textbf{LLM-Personalize(\si2)} & 4.52 & 1.92 & \textbf{6.32} & {\ul 1.39} & 5.80 & 3.00 & 6.93 & 4.10 & 7.12 & 3.12 & 7.34 & 3.62 & 4.60 & 3.24 & \textbf{5.53} & 3.68 \\ \bottomrule
\end{tabular}
    \label{table:correct_wrong}
\end{table}

==> table_cross_domain.tex <==
\begin{table}[t]
\caption{Ablation Study: Cross-domain generalisation success rate. (\textbf{Boldface}: best across the task set, \textbf{\si1/2}: self-training iteration 1 or 2, \textbf{\il{}}: imitation learning)}
    \footnotesize
    \setlength\tabcolsep{1pt}
    \hspace*{-0.4cm}
    \begin{tabular}{@{}cllll@{}}
\toprule
\textbf{Scene Pairs} & \multicolumn{2}{c}{\textbf{Scene 1 \& 2}} & \multicolumn{2}{c}{\textbf{Scene 3 \& 4}} \\ \midrule
\textbf{Task Set} & \multicolumn{1}{c}{\textit{\textbf{test(Scene1)}}} & \multicolumn{1}{c}{\textit{\textbf{train(Scene2)}}} & \multicolumn{1}{c}{\textit{\textbf{test(Scene3)}}} & \multicolumn{1}{c}{\textit{\textbf{train(Scene4)}}} \\ \midrule
\textbf{LLM-Planner} & -3.60 ± 4.86 & -8.40 ± 3.84 & -4.07 ± 3.39 & -29.60 ± 5.26 \\ \midrule
\textbf{LLM-Personalize(\il)} & 13.20 ± 6.55 & -3.38 ± 3.08 & 34.33 ± 5.40 & 10.93 ± 3.32 \\ \midrule
\textbf{LLM-Personalize(\si1)} & 13.00 ± 4.68 & \textbf{19.48 ± 2.99} & 31.26 ± 4.91 & 24.23 ± 3.28 \\ \midrule
\textbf{LLM-Personalize(\si2)} & \textbf{17.00 ± 4.59} & 18.52 ± 2.66 & \textbf{42.47 ± 3.86} & \textbf{29.15 ± 2.90} \\ \bottomrule
\end{tabular}
    \label{table:cross_domain}
\end{table}

==> table_discovery.tex <==
\begin{table}[t]
\setlength\tabcolsep{1.0pt}
\footnotesize
\caption{Ablation: Average number of receptacles discovered per episode ((\textbf{Boldface}: best variant across the task set, \textbf{SI}: self-imitation, \textbf{IL}: imitation learning)}
\centering
\begin{tabular}{@{}cllllllll@{}}
\toprule
\textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \midrule
\textbf{task set} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} \\ \midrule
\textbf{LLM-Planner} & 54.20 & 47.24 & 32.32 & 35.84 & 16.84 & 16.00 & 23.84 & 26.56 \\ \midrule
\textbf{LLM-Personalize(\il{})} & 54.52 & 50.59 & 36.84 & \textbf{40.17} & \textbf{18.16} & 17.15 & \textbf{24.08} & 29.03 \\ \midrule
\textbf{LLM-Personalize(\si1)} & \textbf{54.60} & \textbf{50.66} & 36.60 & 39.50 & 17.32 & \textbf{17.53} & \textbf{24.08} & \textbf{29.12} \\ \midrule
\textbf{LLM-Personalize(\si2)} & 54.56 & 50.60 & \textbf{37.40} & 39.49 & 16.92 & 16.90 & 23.92 & 28.70 \\ \bottomrule
\end{tabular}
\label{table:discovered_recs}
\end{table}

==> table_executability.tex <==
\begin{table}[t]
\setlength\tabcolsep{1.5pt}
\caption{Ablations: Executability - percentage of successfully executed steps (\textbf{Boldface}: best variant across the task set, \textbf{SI}: self-imitation, \textbf{IL}: imitation learning)}
    \centering
\begin{tabular}{@{}cllllllll@{}}
\toprule
\textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \midrule
\textbf{task set} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} \\ \midrule
\textbf{LLM-Planner} & 74.17 & 73.73 & 77.53 & 82.34 & 78.36 & 81.84 & 76.12 & 79.91 \\ \midrule
\textbf{LLM-Personalize (\il{})} & \textbf{93.00} & \textbf{91.86} & \textbf{96.05} & \textbf{94.43} & 89.00 & 86.32 & \textbf{95.51} & 93.44 \\ \midrule
\textbf{LLM-Personalize (\si1)} & 90.12 & 89.02 & 88.01 & 92.65 & \textbf{91.32} & 89.39 & 92.50 & \textbf{95.35} \\ \midrule
\textbf{LLM-Personalize (\si2)} & 87.58 & 89.84 & 95.25 & 93.76 & 90.59 & \textbf{93.57} & 90.27 & 92.31 \\ \bottomrule
\end{tabular}
    \label{table:executability}
\end{table}

==> table_main.tex <==
\begin{table*}[t]
\caption{Average success rate on train and test sets across scenes. Each entry denotes the mean ± standard error of the mean across multiple episodes. (\textbf{Boldface}: best variant across the task set, \textbf{\si{}}: self-training, \textbf{\il{}}: imitation learning)}
    \centering
    \footnotesize
    \setlength\tabcolsep{1pt}
\begin{tabular}{@{}ccllllllll@{}}
\toprule
\multicolumn{1}{l}{\textbf{}} & \textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \cmidrule(l){2-10} 
\multicolumn{1}{l}{} & \textbf{Task Set} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} \\ \midrule
\multirow{3}{*}{\textbf{Baselines}} & \textbf{SayCan} & 0.00 ± 0.00 & -2.67 ± 1.90 & -10.67 ± 6.86 & -1.25 ± 1.25 & -8.00 ± 4.90 & -3.33 ± 2.29 & 0.00 ± 0.00 & -1.67 ± 1.67 \\ \cmidrule(l){2-10} 
 & \textbf{SayPlan} & -5.00 ± 5.00 & -7.00 ± 5.91 & -1.67 ± 9.28 & -6.83 ± 2.78 & -13.00 ± 8.31 & 0.42 ± 4.50 & -12.33 ± 15.34 & -10.75 ± 3.89 \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Planner} & -3.60 ± 4.86 & 5.33 ± 4.44 & -9.87 ± 6.35 & -8.40 ± 3.84 & -4.07 ± 3.39 & -14.27 ± 4.00 & -30.27 ± 4.84 & -29.60 ± 5.26 \\ \midrule
\multirow{3}{*}{\textbf{Ours}} & \textbf{LLM-Personalize (\il{})} & 17.60 ± 6.17 & 4.17 ± 2.63 & 12.60 ± 9.07 & -3.38 ± 3.08 & 24.33 ± 4.41 & 22.62 ± 2.64 & \textbf{25.73 ± 6.78} & 10.93 ± 3.32 \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Personalize (\si{} \ione{})} & 25.80 ± 6.69 & 17.98 ± 3.79 & 21.73 ± 5.63 & \textbf{19.48 ± 2.99} & 41.40 ± 6.35 & 32.42 ± 3.20 & 10.27 ± 6.71 & 24.23 ± 3.28 \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Personalize (\si{} \itwo{})} & \textbf{29.60 ± 5.40} & \textbf{25.52 ± 3.14} & \textbf{25.20 ± 4.05} & 18.52 ± 2.66 & \textbf{43.33 ± 4.35} & \textbf{33.58 ± 3.85} & 20.40 ± 6.82 & \textbf{29.15 ± 2.90} \\ \bottomrule
\end{tabular}
%\end{tabularx}
    \label{table:main_results}
\vspace{-5mm}
\end{table*}

==> table_main_reduced.tex <==
\begin{table*}[t]
\caption{Average success rate on train and test sets across scenes. Each entry denotes the mean ± standard error of the mean across multiple episodes. (\textbf{Boldface}: best variant across the task set, \textbf{\si{}}: self-training, \textbf{\il{}}: imitation learning)}
    \centering
    %\footnotesize
    \setlength\tabcolsep{3pt}
    \begin{tabular}{@{}cccccccccc@{}}
\toprule
\textbf{} & \textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \midrule
 & \textbf{Task Set} & \textit{\textbf{train}} & \textit{\textbf{test}} & \textit{\textbf{train}} & \textit{\textbf{test}} & \textit{\textbf{train}} & \textit{\textbf{test}} & \textit{\textbf{train}} & \textit{\textbf{test}} \\ \midrule
\multirow{3}{*}{\textbf{Baselines}} & \textbf{SayCan} & -2.6 ± 1.9 & 0.0 ± 0.0 & -1.2 ± 1.2 & -10.6 ± 6.8 & -3.3 ± 2.2 & -8.0 ± 4.9 & -1.6 ± 1.6 & 0.0 ± 0.0 \\ \cmidrule(l){2-10} 
 & \textbf{SayPlan} & -7.0 ± 5.9 & -5.0 ± 5.0 & -6.8 ± 2.7 & -1.6 ± 9.2 & 0.4 ± 4.5 & -13.0 ± 8.3 & -10.7 ± 3.8 & -12.3 ± 15.3 \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Planner} & 5.3 ± 4.4 & -3.6 ± 4.8 & -8.4 ± 3.8 & -9.8 ± 6.3 & -14.2 ± 4.0 & -4.0 ± 3.3 & -29.6 ± 5.2 & -30.2 ± 4.8 \\ \midrule
\multirow{3}{*}{\textbf{Ours}} & \textbf{LLM-Personalize (\il{})} & 4.1 ± 2.6 & 17.6 ± 6.1 & -3.3 ± 3.0 & 12.6 ± 9.0 & 22.6 ± 2.6 & 24.3 ± 4.4 & 10.9 ± 3.3 & \textbf{25.7 ± 6.7} \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Personalize (\si{} \ione{})} & 17.9 ± 3.7 & 25.8 ± 6.6 & \textbf{19.4 ± 2.9} & 21.7 ± 5.6 & 32.4 ± 3.2 & 41.4 ± 6.3 & 24.2 ± 3.2 & 10.2 ± 6.7 \\ \cmidrule(l){2-10} 
 & \textbf{LLM-Personalize (\si{} \itwo{})} & \textbf{25.5 ± 3.1} & \textbf{29.6 ± 5.4} & 18.5 ± 2.6 & \textbf{25.2 ± 4.0} & \textbf{33.5 ± 3.8} & \textbf{43.3 ± 4.3} & \textbf{29.1 ± 2.9} & 20.4 ± 6.8 \\ \bottomrule
\end{tabular}
% \begin{tabular}{@{}ccllllllll@{}}
% \toprule
% \multicolumn{1}{l}{\textbf{}} & \textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \cmidrule(l){2-10} 
% \multicolumn{1}{l}{} & \textbf{Task Set} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} \\ \midrule
% \multirow{3}{*}{\textbf{Baselines}} & \textbf{SayCan} & 0.0 ± 0.0 & -2.6 ± 1.9 & -10.6 ± 6.8 & -1.2 ± 1.2 & -8.0 ± 4.9 & -3.3 ± 2.2 & 0.0 ± 0.0 & -1.6 ± 1.6 \\ \cmidrule(l){2-10} 
%  & \textbf{SayPlan} & -5.0 ± 5.0 & -7.0 ± 5.9 & -1.6 ± 9.2 & -6.8 ± 2.7 & -13.0 ± 8.3 & 0.4 ± 4.5 & -12.3 ± 15.3 & -10.7 ± 3.8 \\ \cmidrule(l){2-10} 
%  & \textbf{LLM-Planner} & -3.6 ± 4.8 & 5.3 ± 4.4 & -9.8 ± 6.3 & -8.4 ± 3.8 & -4.0 ± 3.3 & -14.2 ± 4.0 & -30.2 ± 4.8 & -29.6 ± 5.2 \\ \midrule
% \multirow{3}{*}{\textbf{Ours}} & \textbf{LLM-Personalize (\il{})} & 17.6 ± 6.1 & 4.1 ± 2.6 & 12.6 ± 9.0 & -3.3 ± 3.0 & 24.3 ± 4.4 & 22.6 ± 2.6 & \textbf{25.7 ± 6.7} & 10.9 ± 3.3 \\ \cmidrule(l){2-10} 
%  & \textbf{LLM-Personalize (\si{} \ione{})} & 25.8 ± 6.6 & 17.9 ± 3.7 & 21.7 ± 5.6 & \textbf{19.4 ± 2.9} & 41.4 ± 6.3 & 32.4 ± 3.2 & 10.2 ± 6.7 & 24.2 ± 3.2 \\ \cmidrule(l){2-10} 
%  & \textbf{LLM-Personalize (\si{} \itwo{})} & \textbf{29.6 ± 5.4} & \textbf{25.5 ± 3.1} & \textbf{25.2 ± 4.0} & 18.5 ± 2.6 & \textbf{43.3 ± 4.3} & \textbf{33.5 ± 3.8} & 20.4 ± 6.8 & \textbf{29.1 ± 2.9} \\ \bottomrule
% \end{tabular}
%\end{tabularx}
    \label{table:main_results}
\vspace{-3mm}
\end{table*}

==> table_scene.tex <==
\begin{table}[h]
\setlength\tabcolsep{1.5pt}
\caption{Rooms in the Tested Scenes}
    \centering
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Scene 1} & \textbf{Scene 2} & \textbf{Scene 3} & \textbf{Scene 4} \\ \midrule
\begin{tabular}[c]{@{}c@{}}kitchen, living room, \\ corridor, bathroom, \\ utility room, \\ pantry room\end{tabular} & \begin{tabular}[c]{@{}c@{}}kitchen, living room, \\ dining room, \\ child's room, \\ bathroom, bedroom\end{tabular} & \begin{tabular}[c]{@{}c@{}}corridor, \\ bathroom, \\ bedroom\end{tabular} & \begin{tabular}[c]{@{}c@{}}kitchen, \\ living room, \\ bathroom, \\ bedroom, lobby\end{tabular} \\ \bottomrule
\end{tabular}
    \label{table:scene_layout}
\end{table}

==> table_unique_placements.tex <==
\begin{table}[t]
\setlength\tabcolsep{1.5pt}
\caption{Ablations: Exploration vs. Exploitation - number of unique placements executed (\textbf{Boldface}: best variant across the task set, \textbf{SI}: self-imitation, \textbf{IL}: imitation learning)}
    \centering
\begin{tabular}{@{}cllllllll@{}}
\toprule
\textbf{Scene ID} & \multicolumn{2}{c}{\textbf{Scene 1}} & \multicolumn{2}{c}{\textbf{Scene 2}} & \multicolumn{2}{c}{\textbf{Scene 3}} & \multicolumn{2}{c}{\textbf{Scene 4}} \\ \midrule
\textbf{task set} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} & \multicolumn{1}{c}{\textit{\textbf{test}}} & \multicolumn{1}{c}{\textit{\textbf{train}}} \\ \midrule
\textbf{LLM-Planner} & 4.00 & 3.68 & 3.84 & 3.28 & 4.76 & 5.44 & 3.96 & 4.08 \\ \midrule
\textbf{LLM-Personalize (\il{})} & 4.24 & 2.89 & \textbf{4.60} & \textbf{5.03} & 2.32 & 2.44 & 7.00 & 4.73 \\ \midrule
\textbf{LLM-Personalize (\si1)} & \textbf{5.28} & \textbf{3.75} & 4.12 & 4.82 & \textbf{9.48} & \textbf{9.17} & \textbf{7.08} & \textbf{6.72} \\ \midrule
\textbf{LLM-Personalize (\si2)} & 4.04 & 2.98 & 4.48 & 4.60 & 8.24 & 7.64 & 6.60 & 6.27 \\ \bottomrule
\end{tabular}
\label{table:unique_placements}
\end{table}
